Measurement of the ttbar production cross section in ppbar collisions at sqrt{s} = 1.96 TeV using kinematic characteristics of lepton + jets events

We present a measurement of the top quark pair production cross section in ppbar collisions at sqrt(s)=1.96 TeV utilizing 425 pb-1 of data collected with the D0 detector at the Fermilab Tevatron Collider. We consider the final state of the top quark pair containing one high-pT electron or muon and at least four jets. We exploit specific kinematic features of ttbar events to extract the cross section. For a top quark mass of 175 GeV, we measure sigma_ttbar = 6.4 +1.3-1.2(stat} +/- 0.7(syst)+/- 0.4(lum) pb in good agreement with the standard model prediction.

==> data.tex <==
\subsection{Data sample}

In this analysis data recorded by the {\dzero} detector between August
2002 and August 2004 is analyzed. The quality of the data used in the 
analysis is ensured by applying
data quality criteria at the run, luminosity block (LBN) and single
event level.

The selection of good runs is based on the information stored in \dzero Run 
Quality Database. It guarantees that no known hardware failures
occurred during the run, possibly corrupting the data, for all detector
systems of importance to this analysis. 

Individual events are rejected if they demonstrate abnormal features such as
very high occupancy in the calorimeter or, on the contrary, no data.    

